Efficient Hardware Primitives for Immediate Memory Reclamation in Optimistic Data Structures

Safe memory reclamation (SMR) algorithms are crucial for preventing use-after-free errors in optimistic data structures. SMR algorithms typically delay reclamation for safety and reclaim objects in batches for efficiency. It is difficult to strike a balance between performance and space efficiency. Small batch sizes and frequent reclamation attempts lead to high overhead, while freeing large batches can lead to long program interruptions and high memory footprints. An ideal SMR algorithm would forgo batching, and reclaim memory immediately, without suffering high reclamation overheads. To this end, we propose Conditional Access: a set of hardware instructions that offer immediate reclamation and low overhead in optimistic data structures. Conditional Access harnesses cache coherence to enable threads to efficiently detect potential use-after-free errors without explicit shared memory communication, and without introducing additional coherence traffic. We implement and evaluate Conditional Access in Graphite, a multicore simulator. Our experiments show that Conditional Access can rival the performance of highly optimized and carefully tuned SMR algorithms while simultaneously allowing immediate reclamation. This results in concurrent data structures with similar memory footprints to their sequential counterparts.

==> sections/abstract.tex <==
\begin{abstract}
Main task of a safe memory reclamation algorithm is to determine and mitigate a problematic case wherein threads could be accessing a concurrently freed shared object which could lead to \emph{use-after-free} errors. Existing algorithms for linked data structures require space and time sub-optimal book-keeping mechanisms to determine the case. Further, the freeing of unlinked object is delayed by amortizing the reclamation over multiple operations to maintain good speedup.

We propose hardware based reclamation (HBR): a set of instructions to design concurrent data structures with safe memory reclamation. HBR reconciles the trade-off between speedup and immediate reclamation. It achieves this by leveraging the underlying cache coherence mechanism which readily provides the information about the probable event where a thread might attempt to access a concurrently freed node, therefore eliminating the need of redundant and sub-optimal book-keeping at the application level.

The technique is easy to program, incurs no extra space at the programming level, is comparable to well known epoch based techniques in terms of speed, and at the same time achieves immediate memory reclamation enabling immediate memory reuse to keep memory footprint comparable to their sequential counterparts. 
\end{abstract}


==> sections/contribution.tex <==
\textbf{Contribution:}
We propose semantics and possible hardware implementation of \textit{Conditional Access}: a set of primitives that enable immediate yet efficient reclamation in concurrent data structures. The aforementioned mechanism is simulated on Graphite multicore simulator\cite{miller2010graphite}. Further, we design a mini benchmark consisting of several data structures and rival memory reclamation algorithms to evaluate \textit{Conditional Access}.
Our technique bridges the abstraction gap between hardware and software providing non trivial performance opportunities. 
It also shows that memory reclamation could be considered as the integral part of concurrent data structure design process rather than a separate module which requires explicit synchronization. 

==> sections/core_idea.tex <==
\textbf{Intuitive explanation of the core idea in HMR:}
Next, the core idea that works underneath the proposed solution is explained by looking at the problem of memory reclamation using the first principles on a lazylist.

Threads in a lazylist consists of a synchronization free \emph{traversal phase} followed by an atomic \emph{update phase}. In the {traversal phase} a thread travels from one node to another using pointers until it reaches the neighbourhood where it executes the intended operation by either simply returning the presence of a node, if it is a lookup operation, or switching to the \emph{update phase}, if the operation is an update. 
Further, if the update operation is a delete and the node is found then it is marked, unlinked and then sent to a memory reclamation module.

Here, all a memory reclamation module cares about is that whenever it frees the node no other thread should hold reference to this node so that \emph{use-after-free} error could be prevented. \todo{Do we need to establish why a use-after-free memory access is bad?} So a memory reclamation module is fundamentally interested in knowing that whenever it wants to free a node whether there is any thread holding a reference to it or not. We posit that any attempt to know this information at application level is redundant as this information is readily available at the architectural level which can be harnessed using software-hardware co-design.

To understand how, let us dig deeper into what happens at architectural level whenever a node is logically marked for deletion. Considering a hypothetical concurrent execution of a thread T1 at core C1 and T2 at core C2 on a lazylist\footnote{ \textcolor{green}{TBD: an exemplary list diagram}}. Say, T1 executes delete(k2) and T2 executes lookup(k2). Now at the moment T1 arrives at k2, C1 fetches k2's address in its L1 cache in \emph{shared(S)} state. Similarly, when T2 arrives at k2, C2 also gets k2's address in its L1 cache in the \emph{shared(S)} state. Later when T1 marks k2 for deletion C1 upgrades k2's cacheline to \emph{modified(M)} state \emph{invalidating(I)} cachelines containing k2 at any other core, in this case T2's cacheline containing k2 in \emph{shared(S)} state is \emph{invalidated(I)}. 

Clearly, if T2 could somehow harness the L1 cache messages then it can learn that T1 has marked k2 for deletion and therefore it can simply avoid accessing the probably freed node k2 without requiring a redundant mechanism (book-keeping) at the software level to learn the same information.
\footnote{readers may try dimissing the idea as very similar to HTM, clarify to readers how we are different than HTM} \footnote{\textcolor{green}{TBD : convey the possibility of false conflict like problem - any update other than logical marking will also cause read restarts. This could be left to \textbf{future work} where we optimize HMR further by fixing false reader-reclaimer conflicts}}      

In related art some mechanisms which exploit the implicit book-keeping ability of cache coherency protocols to design concurrent data structure exist like hardware transactional memory, load-linked and store conditional pair and Memory Tagging\cite{alistarh2020memory}. However, it is not obvious how efficient data structures supporting safe memory reclamation could be designed \textemdash either they introduce complexity in the existing data structures or could not directly be used because of their restricted properties. In order to fix this, our work builds upon Alistarh and Brown's\cite{alistarh2020memory} MemoryTagging to propose a set of instructions to design concurrent data structures with safe memory reclamation. HBR, similar to the aforementioned techniques, leverages coherence protocol to make immediate reclamation based concurrent data structures easier and faster.  

==> sections/correct-short.tex <==
\section{Correctness}
\label{sec:corr}

\begin{assumption}
Programs are well behaved \textit{i.e.} they call provided HBR API appropriately.
\begin{enumerate}
    \item reader/writer rule is followed.
    \item reclaimer rule is followed that is a thread unlinks a node, marks it and then frees it.
    \item only one thread could free a node.
\end{enumerate}
\label{asm:wellbehave}
\end{assumption}

For HBR based programs to be correct, all data structure operations should do shared memory reads and writes using \crd{} and \cwr{} and a thread is required to write on a node before freeing it. 

Additionally, for \textit{reader-writer} rule to work we assume that the underlying hardware provides cache coherency mechanism like MSI, MESI or other such equivalent mechanism. 

\begin{property}
\label{prop:cAccessAtomic}
\crd{} and \cwr{} instructions atomically:
    tag a node on its first access and conditionally access the node. Access is a read if \crd{} is executing else the access is a write for \cwr{}.
\end{property}

Henceforth, we will refer to \crd{} and \cwr{} as \textit{conditional access}.

\begin{property}
\label{prop:cAccessSucc}
A conditional access only succeeds if none of the tagged locations have been invalidated since they were tagged
\end{property}

\begin{property}
\label{prop:writeinvalidates}
When a memory location is written the cache coherency mechanism invalidates all the cached copied of the location at other threads, thus if the location is tagged at the other threads, then these tags are also invalidated.
\end{property}

\begin{property}
\label{prop:spurious}
A conditional access can fail spuriously but it will never succeed spuriously.
\end{property}

\begin{lemma}
\label{lemma:correcttag}
In a correctly synchronized data structure if all regular accesses are replaced by conditional accesses then a node is guaranteed to be reachable in data structure at the time it is tagged. 
\end{lemma}

We prove this lemma for the case where no nodes are untagged. However it can be extended to the case where only a small set of nodes are tagged and previously tagged nodes which are no longer needed are untagged. This will be similar, in spirit, to hand-over-hand locking where only a small set of nodes are needed to be locked at a time to ensure traversals are correct.
\begin{proof}
Consider a sequence of linked nodes in a data structure reachable from a sentinel node \textit{head}, which is never deleted, and where all reads are replaced by \crd{s}.
For ease in exposition we ignore spurious failure which anyways concerns progress and not the correctness.
% : head $\longrightarrow$ $n_1$ $\longrightarrow$ $n_2$ $\cdots$ $\longrightarrow$ $n_k$. 
\\
\\
\noindent
\textbf{base case:}
The \head is never deleted so when it is tagged it is reachable in the data structure. Typically head will be \crd{} which atomically: tags address of head and then conditionally reads a value in \head (\propref{cAccessAtomic}). Upon success head is assigned to a local pointer. Since the \crd{} is atomic the conditional read is guaranteed to succeed.

The first node (pointed to by \head) is tagged when any of its fields are accessed (\crd{}) by dereferencing the local pointer. Note, this \crd{} will only succeed if the \head was not modified since it was tagged. Thus, the first node is guaranteed to be reachable from head at the time it is tagged, otherwise the \crd{} will fail and the operation will restart.
\\
\\
\noindent
\textbf{Induction hypothesis:}
Lets say, at some time we have successfully \crd{} next field of some $i_{th}$ node, named \pred in a local pointer \curr. Such that all nodes from \head to \pred were reachable at the time they were tagged. Now, we are about to read a field of \curr (dereference) upon which it will also be tagged. We shall show that \curr is guaranteed to be reachable at the time it would be \crd{} by this way.

Note, \curr could only be made unreachable from head by unlinking, which will require modifying the next field of \pred{}.

Also from \propref{cAccessAtomic} and \propref{cAccessSucc} we know that upon a \crd{} a location is tagged and then fate of access is decided based on the condition that none of the tagged locations have been invalidated. If the condition fails then all locations are untagged and the operation is retried. Therefore, when a field of \curr{} is \crd{} then the node pointed to by \curr will be tagged atomically followed by the validation of all the currently tagged location. If \curr was unlinked then \pred{'s} next field would have changed which would cause invalidation of the tagged \pred node. This would cause \crd{} on \curr to fail removing all tags and restarting the operation. Thus, if the \crd succeeds then it is guaranteed that \curr has not been unlinked.
\end{proof}

% \begin{lemma}[HBR is Safe]
% \label{lem:hbrsafe}
% Threads will never dereference a freed node. In other words, a \crd{} will fail if a node has been freed since it was last accessed. 
% \end{lemma}
% \begin{proof}
% Lets assume, that HBR is unsafe, thus a thread could dereference a freed node. And for this to happen, 
% (P): a conditional access on a freed node \textit{n} by some thread $T_i$ must succeed.
% Assuming, P is true. That is a conditional access on \textit{n} by $T_i$ succeeds even though \textit{n} has been freed, by some thread $T_j$, since it was last tagged during its first access by $T_i$.

% Lets say, $T_j$ frees \textit{n} at time $t_f$. $T_i$ first conditionally accesses and thus tags \textit{n} and again conditionally access (to dereference) it at time $t_t$ and $t_d$, respectively. Such that, $t_t$ $<$ $t_f$ $<$ $t_d$.

% From reclaimers rule, we know that, to free a node a thread: unlinks, writes, and then frees it. And, from \propref{writeinvalidates} we know that whenever a node is written upon, the remote tagged copies of the node are invalidated. Thus, when $T_j$ frees \textit{n} it unlinks it (modifies pred) and then marks it. And this marking causes the tag of \textit{n} at $T_i$ to be invalidated. Since the tag of $T_i$ has been invalidated, the subsequent conditional access at the time $t_d$ will fail. This contradicts our assumption (P) that the \crd{} at time $t_d$ succeeds. Implying, a \crd{} can never access a freed node. Thus, HBR is safe.
% \end{proof}

\begin{theorem}[HBR is Safe]
\label{thm:hbrsafe}
If a node was reachable in its data structure at the time it was tagged then any subsequent conditional access will never succeed if the node has been freed since it was tagged.
\end{theorem}
In other words, given nodes are tagged appropriately then a \crd{} will never access a freed node. On way of ensuring that nodes are correctly tagged is replacing all reads of shared memory location by \crd{s} and explicitly untagging any previous nodes which would not be required to establish the reachability of current or future nodes. 
\begin{proof}

Lets assume the contrary, that is some thread succeeds a conditional access on a node which was freed since the thread tagged it.
Say, $T_i$ tags \textit{n} and again conditionally access (to dereference) it at time $t_t$ and $t_d$, respectively. $T_j$ frees \textit{n} at time $t_f$. Such that, $t_t$ $<$ $t_f$ $<$ $t_d$.

From reclaimers rule, we know that, to free a node a thread: writes and then frees it. And, from \propref{writeinvalidates} we know that whenever a node is written upon, the remote tagged copies of the node are invalidated. 

Thus, when $T_j$ marks \textit{n} before freeing it. This marking causes the tag of \textit{n} at $T_i$ to be invalidated. Since the tag of $T_i$ is invalidated, the subsequent conditional access at the time $t_d$ will fail.

This contradicts our assumption that the \crd{} succeeds on \textit{n} (at time $t_d$) even though the node has been freed (at time $t_f$) since it was tagged (at time $t_t$).

Since, \crd{} cannot fail and succeed at the same time. Our assumption was wrong. Implying, a \crd{} can never access a freed node. Thus, HBR is safe.
\end{proof}

\begin{lemma}[HBR is ABA free] Conditional accesses in HBR are immune to ABA problem.
\label{lem:abasafe}
\end{lemma}
\begin{proof}
Assume, that conditional accesses in HBR based data structure have ABA problem. Therefore, there exists a case where a memory location \textit{m} is conditionally accessed by a thread $T_i$ (A), and then \textit{m} is modified by another thread $T_j$ (B), followed by another conditional memory access on \textit{m} by $T_i$ (A), such that the second memory access succeeds without recognising the fact that \textit{m} was changed since its first access. 

Since, whenever a memory location is first \crd{} it is tagged, $T_i$ tags \textit{m} when it does its first \crd{} on \textit{m}. Later if \textit{m} is modified by $T_j$ then by virtue of the cache coherence mechanism it invalidates all the remote copies of \textit{m}, in process invalidating the tags (\propref{writeinvalidates}). Therefore, when $T_i$ does \crd{} again on \textit{m} it will find that \textit{m} has been invalidated causing it to fail (\propref{cAccessSucc}). Since, a \crd{} cannot fail and succeed at the same time, our initial assumption that the second \crd{} on \textit{m} by $T_i$ succeeds even when another thread modifies it after $T_i$ first accessed it is wrong. Therefore, ABA issue cannot occur.

\end{proof}

\begin{property}[Progress]
\label{prop:hbrprogress}
Searches in HBR based algorithms are guaranteed to be lockfree provided hardware allows no spurious failure.
\end{property}

If HBR instructions are implemented in hardware such that spurious failures due to associativity evictions or interrupts are eliminated and conditional accesses could only fail due to real data conflicts then searches for HBR based data structures could be guaranteed to be lock-free. Because, a failure of a conditional access would imply that some thread successfully executed an update on a conflicting address and thus at least one thread is guaranteed to make progress.

On the other hand, if the implementation of proposed HBR semantics could not guarantee freedom from spurious failures then a fallback technique could be used. 
\\
\\
\noindent
\textbf{facilitating progress}
As noted conditional accesses are vulnerable to spurious failures due to limits on hardware resources, like overflow of tagged cachelines because of associativity evictions. To reduce the probabilty of such spurious failures we propose \utag{} which helps in maintaining only a minimal set of tagged references by untagging previous locations which will not be required to establish correctness of searches.

<<anchor based lock acquisition idea where we can untag all previous nodes once first lock is acquired>> 



==> sections/correctness.tex <==
\section{Correctness}
\label{sec:corr}

For \ca based programs to be correct, all data structure operations should do shared memory reads and writes using \crd{} and \cwr{} and a thread is required to write on a node before freeing it. 

Additionally, for \textit{reader-writer} rule to work we assume that the underlying hardware provides cache coherency mechanism like MSI, MESI or other such equivalent mechanism. 

\begin{lemma}
\label{lemma:correcttag}
In a correctly synchronized data structure if all regular accesses are replaced by conditional accesses then a node is guaranteed to be reachable in data structure at the time it is tagged. 
\end{lemma}

\begin{theorem}[\ca is Safe]
\label{thm:hbrsafe}
If a node was reachable in its data structure at the time it was tagged then any subsequent conditional access will never succeed if the node has been freed since it was tagged.
\end{theorem}

\begin{lemma}[\ca is ABA free] Conditional accesses in \ca are immune to ABA problem.
\label{lem:abasafe}
\end{lemma}

\begin{property}[Progress]
\label{prop:hbrprogress}
Searches in \ca based algorithms are guaranteed to be lockfree provided hardware allows no spurious failure.
\end{property}


==> sections/incorrectlistimplwithCA.tex <==
% Nevertheless, simple data structures, like VAS-based linked list\textemdash a MemoryTagging based variant of harris list \cite{harris2001pragmatic}, can be designed for immediate reclamation using HBR.
% We will see through simple data structure to see kinds of challenges that could occur in using HBR.

% - VAS based linked list. Delete: mark and then unlink-free. In case mark succeeds and unlink fails let searches unlink.

% - Search in VAS list : if find a marked node. first have to unlink it. 


% \begin{algorithm}[h]
%     \caption{Using HBR with VAS-based List. Incorrect Implementation}
%     \label{algo:vaslist}
%     \footnotesize
%     \begin{algorithmic}[1]
%         \State type Node \{Key key, lock, mark, Node *next\}
%         \State class list \{Node *head\}

%         \Procedure{locate}{Key key}
%             \State retry:
%             \State pred $\leftarrow$ \crdp{head}
%             \State curr $\leftarrow$ \crdp{pred->next} if $\bot$ \utagall{} \& retry
%             \State currkey $\leftarrow$ \crdp{curr->key}  if $\bot$ \utagall{} \& retry
%             \While{currkey < key}
%                 \State \utag{pred}
%                 \State pred $\leftarrow$curr                
%                 \State curr $\leftarrow$ \crdp{pred->next} if $\bot$ \utagall{} \& retry

%                 \State currmark $\leftarrow$ \crdp{curr->mark} if $\bot$ \utagall{} \& retry
%                 \If{$currmark$}
%                     \State succ $\leftarrow$ \crdp{curr->next} if $\bot$ \utagall{} \& retry
%                     \If {False == \texttt{\cwrp{pred->next}{succ}}}
%                         \State \texttt{untagAll() and goto retry}
%                     \EndIf
%                     \State free(curr) 
%                     \State curr $\leftarrow$ succ                
%                     % \State \texttt{untagAll() and goto retry} \Comment{succ may not be }
%                 \EndIf
%                 \State currkey $\leftarrow$ \crdp{curr->key}  if $\bot$ \utagall{} \& retry
%             \EndWhile
%         \EndProcedure
%         \Statex
%         \Procedure{contain}{key}
%             \State $\langle$ pred, curr, currkey $\rangle$ $\leftarrow$ locate(key)
%             \State \utagall{}
%             \State return (currkey == key)
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}        

% \begin{algorithm}
%     \caption{Delete in VAS-based List.}
%     \label{algo:vaslistdel}
%     \footnotesize
%     \begin{algorithmic}[1]
%         \Procedure{delete}{key}
%             \State retry:
%             \State $\langle$ pred, curr, currkey $\rangle$ $\leftarrow$ locate(key)
%             \If{currkey != key}
%                 \State \utagall{} \& return False
%             \EndIf
%             \If {False == \texttt{\cwrp{curr->mark}{1}}}
%                 \State \texttt{untagAll() and goto retry}
%             \EndIf
%             \If {False == \texttt{\cwrp{pred->next}{curr->next}}}
%                 \State \texttt{untagAll() and goto retry}
%             \EndIf
%             \utagall{}
%             \State free(curr)
%             \State return True
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

==> sections/specandimpl.tex <==
\section{Proposed Technique}
\label{sec:hmr}
% HMR leverages MemoryTag's ability to harness cache level messages to know whether a cacheline has been invalidated since its previous access. This indirectly, when a node is marked logical deletion at the application level, the corresponding core invalidates the cacheline of other cores containing the node's address at the cache level. If we can harness these cache messages then a core whose cacheline has been invalidated since its previous access could reasonably assume that the node might have been deleted. Therefore, solving the issue of safely accessing a memory location. MemoryTags exactly does this. It allows threads to tag a set of locations before accessing them, read them, and later validate. The validate succeeds if the tagged memory locations have not been modified since they were last tagged. At the cache level meaning that no other core has invalidated the cacheline. Otherwise the validation fails.

% In the proposed memory reclamation technique, intuitively, a thread reading a memory location and a thread trying to reclaim the location do a mutual handshake. A thread reclaiming a memory location has to do a write (mark the node), so that caches of other cores could be invalidated. And a thread attempting to read a memory location guarantees to first tag it, then validate, and then if validation succeeds reads it. This way safe memory reclamation is achieved.   

HBR observes the L1 cache level events that allow safe use of references in presence of concurrent deletes.

\textbf{Reclaimer side behaviour:} Any thread that wants to free a node does a write on the node by setting mark bit of the node (logical deletion) and then frees it. At the cache level, writing on the node causes cache coherence protocol to send invalidation messages to the cores that might have the node in their L1 cache. The cores which receive the invalidation request adds the address in a core local \emph{EvictSet} data structure. This means any thread which might have a reference to this node, by monitoring these invalidation messages, could learn that the node might be concurrently freed. 

\textbf{Reader side behaviour:} A thread that intends to access a memory location first tags it and then accesses it. Tagging is way to start observing  for any invalidation messages at the corresponding core's L1-cache. It is done by adding the address in a core local \emph{TagSet} data structure. Only after an address is tagged threads could access the content at the memory location. Accessing the memory location involves the use of atomic \emph{vRead} and \emph{vWrite} (short for validate and read or validate and write). Validate checks whether a cacheline received any invalidation request since the corresponding address was added to the \emph{TagSet}. If that is true, the validation fails and the subsequent memory access operation (read or write) is skipped, otherwise thread could safely do subsequent read or write on the tagged memory location. To be more precise \emph{validate} involves checking whether the address in question is present in \emph{EvictSet}. If the thread is certain that it does not require a reference any more it can remove the address from the \emph{TagSet} and the \emph{EvictSet} by invoking \emph{unTag}.

We now discuss the API specification of the proposed Hardware based reclamation technique.
\subsection{API Specification}
\label{sec:spec}

For the simplicity in exposition we assume that each address is aligned to a cacheline size and occupies one cacheline. Thus, an operation on an address should be understood as an operation on its cacheline.\footnote{My readers should not be confused about a mental picture while thinking of what happens at app level how it translates to cachelevel events.}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.4\textwidth]{figs/tvr.pdf}
% \caption{\func{TvRead} specification.}
% \label{fig:tvr}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.4\textwidth]{figs/vwrite.pdf}
% \caption{\func{vWrite} specification.}
% \label{fig:vwrite}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.4\textwidth]{figs/untag.pdf}
% \caption{\func{unTag(X)} and \func{unTagAll} specification.}
% \label{fig:untag}
% \end{figure}

% \begin{figure*}[htbp]
%      \begin{minipage}{\textwidth}
%         \begin{subfigure}{\textwidth}
%             \includegraphics[width=0.45\linewidth, height=6cm, keepaspectratio]{figs/vread.png}\hfill
%             \includegraphics[width=0.45\linewidth, height=6cm, keepaspectratio]{figs/vwrite.png}\hfill
%             \label{fig:vops}
%         \end{subfigure}
%      \end{minipage}
% \vspace*{-3mm}
%     \caption{HBR specification
%     }
%     \label{fig:vrwspec}
% \end{figure*}

\noindent
\textbf{\func{TagSet} and \func{EvictSet}:} These are two data structures that reside at the L1cache level thus are local to each core. \emph{TagSet} maintains the cachelines that are currently tagged and \emph{EvictSet} maintains the cachelines which have been invalidated/flushed since they were last tagged. These two data structures together help HBR to keep track of coherence protocol's messages to learn when a tagged cacheline might have been invalidated possibly due to a deletion at the common address in some other core. For example, when an address is present in a core's \emph{TagSet} and is also present in the core's \emph{EvictSet} then it could infer that the tagged address is not valid anymore due to a concurrent modification elsewhere (possibly a logical deletion). \tabref{ds_states} lists the possible ways a given cacheline could be present in the two data structures and what does that mean for HBR. 
\begin{table}[]
    \centering
    \begin{tabular}{cc|c}
    TagSet & EvictSet & Cacheline State \\
    \hline
    0 & 0 & not applicable \\
    0 & 1 & not applicable \\
    1 & 0 & was tagged \& is still valid \\
    1 & 1 & was tagged \& is not valid \\
    \end{tabular}
    \caption{Interpretation of HBR about a tagged address based on its presence in TagSet and EvictSet.}
    \label{tab:ds_states}
\end{table}

% \noindent
% \textbf{\func{tag(r)}} when at the application level tag() is invoked on a reference $r$ then at the cache-level the core adds the corresponding cacheline in its \emph{TagSet}. This also marks the beginning of monitoring of the cache invalidation messages for the concerned cacheline. Every thread before accessing any memory location has to invoke \emph{tag}. \figref{tagspec} shows the flowchart for the expected behaviour of a tag instruction. 
% \\
% \\
\noindent
\textbf{\func{TvRead(addr)}}, when invoked from a data structure operation on a reference $r$, translates to atomic tagging (if not already tagged earlier) of $r$ and conditional execution of a normal memory \emph{read} operation at the cache level. It returns the status whether it succeeded or failed. The validate fails if both \emph{TagSet} and \emph{EvictSet} contain the cacheline that corresponds to the reference $r$. This means that since the cacheline was last tagged some core has sent invalidation message which has caused addition of the cacheline to the \emph{EvictSet}. So the \emph{read} is skipped and \emph{vRead} returns FAIL. Otherwise, no core has done any modification, including marking the node for logical deletion, since the cacheline was last tagged. Therefore, current \emph{vRead's} \emph{read} will be safe and a valid value at $r$ is returned. Note, we assume that at the time \emph{tag} is invoked the concerned memory location is reachable in data structure and has not been logically deleted. The flowchart in \figref{tvr} demonstrates the working of \func{TvRead}.
\\
\\
\noindent
\textbf{\func{vWrite(addr, v)}}, similar to a \emph{vRead}, when invoked from a data structure operation, translates to an atomic conditional execution of a normal memory \emph{write} of $v$ to $addr$ at the cache level and returns the status whether it succeeded or failed. \emph{vWrite} is same as VAS (an efficient variant of CAS) as proposed in MemoryTagging paper. \figref{vwrite} illustrates the working of the vWrite  operation.

\noindent
\textbf{\func{unTag(addr)} and \func{unTagAll()}} Threads at data structure operation level can invoke \emph{untag} on $addr$ or \emph{untagAll} to remove $addr$ or all the tagged references, respectively, from the \emph{TagSet} and \emph{EvictSet}. \figref{untag} illustrates the expected behaviour of the untag and unTagAll instructions.

% \begin{lstlisting}[mathescape=true, style=ajstyle, caption={HBR sequential Specification.}]
% $T$ = set of all threads.
% $R$ = set of all references in a program.
% $\Phi$ = empty set

% Data structures:
%   TagSet $\mathcal{TS}$ : $T$ $\rightarrow$ $R$, initially $\mathcal{TS}(t)$ $\in$ $\Phi$, $\forall$ $t$ $\in$ $T$ 
%   EvictSet $\mathcal{ES}$ : $T$ $\rightarrow$ $R$, initially $\mathcal{ES}(t)$ $\in$ $\Phi$, $\forall$ $t$ $\in$ $T$

% procedure tag($r:R$) for $r$ $\in$ $R$
%   assert $\&r$ $\notin$ $\mathcal{TS}$
%   $\mathcal{TS}$ $\leftarrow$ $\mathcal{TS}$ $\cup$ $\&r$

% //executes atomically
% function vRead($r:R$) for $r$ $\in$ $R$
%   if $\&r$ $\in$ $\mathcal{TS}$ and $\&r$ $\notin$ $\mathcal{ES}$ //validate
%     return $r$
%   else
%     return FAIL

% //executes atomically
% function vWrite($\&r:R$, $d:R$) for $r$, $d$ $\in$ $R$
%   if $\&r$ $\in$ $\mathcal{TS}$ and $\&r$ $\notin$ $\mathcal{ES}$ //validate
%     $r$ $\leftarrow$ $d$
%     return SUCC
%   else
%     return FAIL

% // A thread that sets a tag only removes its own tag.
% // cannot invoke untag without invoking tag() first.
% procedure untag($r:R$) for $r$ $\in$ $R$
%   assert $\&r$ $\in$ $\mathcal{TS}$
%   $\mathcal{TS}$ $\leftarrow$ $\mathcal{TS}$ $\setminus$ $\&r$
%   $\mathcal{ES}$ $\leftarrow$ $\mathcal{ES}$ $\setminus$ $\&r$

% // A thread that sets a tag only removes its own tag.
% // cannot invoke untag without invoking tag() first.
% procedure untagAll() for $r$ $\in$ $R$
%   assert $\mathcal{TS}$ $\neq$ $\Phi$
%   for each $\&r$ in $\mathcal{TS}$: 
%     $\mathcal{TS}$ $\leftarrow$ $\mathcal{TS}$ $\setminus$ $\&r$
%     $\mathcal{ES}$ $\leftarrow$ $\mathcal{ES}$ $\setminus$ $\&r$    
% \end{lstlisting}

\subsection{Implementation}
\label{sec:impl}
There could be multiple possible hardware implementations that could realize the aforementioned HBR semantics specification.

\subsubsection{Realization 1}

One way to realize the proposed specification is to use a \emph{tag} bit per cacheline. Tagging bit of a cacheline is used to determine whether any conflicting memory access occurs since the cacheline was tagged. A conflicting memory access could be a normal update or logical removal of a node from a shared data structure along with another threads read or update. Two reads on same address from different threads do not conflict. For ease in exposition we assume MSI as the underlying cache coherence protocol where each address is cacheline aligned and occupies the whole cacheline. Additionally we also assume that one thread runs on one core.

% \begin{figure}[h]
% \centering
% \includegraphics[width=4cm]{figs/implsys.pdf}
% \caption{Computer system. LB: Load buffer, SB: Store buffer}
% \end{figure}

\noindent
\textbf{Tagging process:}
If the \emph{tag} instruction is executed from an application code then at the cache level the system first attempts to load the corresponding data from the L1 data cache. If the access causes a hit then the cacheline's tag bit is set. Otherwise in case of a miss, the system fetches the cacheline from higher levels of memory hierarchy and then sets the tag bit in L1 data cache. Note that tagging uses the usual cache transaction that would execute on a regular load instruction. A cacheline remains tagged unless its tag bit is explicity reset by the \emph{untag or untagAll} instruction.
\\
\\
\noindent
\textbf{Untagging process:}
When from a data structure operation \emph{untag} or \emph{untagAll} is executed then the tag bit of the corresponding cacheline is reset. This causes the system to stop monitoring the untagged cachelines for conflicting memory accesses. The \emph{untag} resets the tag bits of the cachelines corresponding to the provided address and the \emph{untagAll} resets tag bits of all the cachelines that were tagged so far in the execution.
\\
\\
\noindent
\textbf{memory access process:}
All read or write (load or store) memory accesses are executed using special \emph{vRead} and \emph{vWrite} instructions. These instructions first validate the provided address for any interfering memory access and then depending upon the result of the validate the intended memory access (load or store) is completed or skipped. The validate mechanism checks whether the cacheline of the provided address has been invalidated or evicted since it was tagged. If the check succeeds that indicates that a conflicting memory access has occured causing the validate to fail. Therefore subsequent memory access should be skipped. Otherwise, the successful validation suggests that no interfering memory access has occurred on the tagged cacheline, meaning, the subsequent memory access is safe. Note that the validate followed by a load or store in vRead or vWrite is an atomic instruction. The vRead/vWrite could fail 1) if the tagged cacheline of the provided address has moved to Invalid state or 2) was evicted due to cache replacement.   

\subsubsection{Realization 2.}

In another variation, the system could maintain two sets, namely a \emph{tagset} and an \emph{evictset} per core at the L1 data cache level. In order to do this, bits in the tag part of the L1 data cachelines could be reserved separately to depict whether a cacheline is tagged (is in tagset) or has been invalidated (is in evictset) since its tag bits were set. This will require that the tagged cachelines are not evicted from the L1 data cache unless explicitly untagged.
\\
\\
\noindent
\textbf{Tagging process:}
Invoking \func{tag} on an address would cause the corresponding cacheline to be loaded in shared state followed by setting the tagset bits. Therefore, priming the system to start monitor for any conflicting memory accesses.
\\
\\
\noindent
\textbf{Untagging process:}
Invoking \func{untag} on a address or \func{untagAll} will reset the tagset and evictset bits of a single cacheline or all the tagged cachelines, respectively. This serves two purposes: 1) releasing the cacheline from being monitored by our system for any interfering traffic and 2) the cacheline could now be allowed to leave L1 data cache. 
\\
\\
\noindent
\textbf{memory access process:}
Major part of any memory access process in our system is to detect the conflicting memory accesses on the tagged cachelines as part of the \emph{vRead} or \emph{vWrite}. This is done using the already existing cache coherence protocol. In particular, whenever a cacheline is modified at a core C1 all its remote copies (at other cores, if any) would be sent an invalidation message. Our system on observing such a message, say at the remote core C2, will set the evictset bits of the cachlines which are in tagset (whose tagset bits are set). Therefore, the validation in any subsequent vRead/vWrite will observe that the cacheline has been sent an evict or invalidate message since it was tagged causing it to fail and retry the operation again hoping for its completion without any interference.

\subsubsection{Realization 3.} 
Another alternative is to utilise the buffers similar to the load buffer on each core between the register file and the l1 data cache to maintain the semantics of tag set and evict set.


==> sections/usage-garbage.tex <==
\section{Using the HBR}
\label{sec:apiuse}
In this section we discuss general rules an user could follow to enable HBR's reclamation in concurrent data structures. Please note that most of the concurrent data structures consist of self-referential node structures where operations could be thought of executing in two phases. First, a read-only traversal phase, and second, an update phase. 

The read only traversal phase involves synchronization-free traversal of the node pointers which stops when some set of destination nodes are identified. The update-phase consists of carrying out the modification of the intended operation on the set of identified nodes, atomically. The atomicity could either be achieved using the synchronization primitives like fine-grained lock based critical sections or Compare-And-Swap.

From the perspective of a reclamation scheme, The important point to note here is that a thread could be envisioned as switching to the read phase when it is finding new references and executing in the update phase when it is operating upon the subset of those references to carry out atomic modifications. We do not make any assumptions on the length of these phases (we see later that stacks have a very short read phase but lazylists have a long read phase).     

We now put forth the the guiding rules which, at broader level, users could follow to integrate HBR in a concurrent data structure.
\begin{enumerate}
    \item \textbf{Readers/Writers rule.} A thread discovering a new reference should first tag and then read/write it using \func{vRead} or \func{vWrite}. Henceforth, referred to as \emph{tag before first access} principle. The point worth mentioning here is that the reference should be reachable from the entry point of the data structure at the moment it is tagged (details in ensuing paragraphs). In other words, all the memory reads/writes vulnerable to \emph{use-after-free} errors should be done using \emph{vRead}/\emph{vWrite}.
    % \item \textbf{Writers rule.} All the memory writes vulnerable to \emph{use-after-free} errors should be done using \emph{vWrite}. Note that the \emph{tag before first access} principle applies for writers too. We mention the writers rule separately to mention that writers 
    \item \textbf{Reclaimers rule.} Threads should write on the node being deleted (precisely, freed).
\end{enumerate}

\noindent
\textbf{Explanation of the rules.}
The \emph{tag-before-access} principle on an address helps readers/writers to learn about the occurrence of any concurrent delete on that address since it was tagged via the status of \func{vRead}/\func{vWrite} instructions. In more detail, upon a tag, HBR starts snooping the cacheline addressed by the node being tagged for any incoming invalidation traffic due to the cache coherence protocol triggered by a concurrent modification elsewhere. And, the subsequent \func{vRead}/\func{vWrite} helps HBR to notify the data structure operation of the possible occurrence of an \emph{use-after-free} error. If the \func{vRead}/\func{vWrite} fails validation then user can interpret that thread might access a freed memory location therefore allowing user to take an alternative action. Possibly restart the operation. Later, when the reference is no more required then it can be untagged which essentially removes the cacheline addressed by the tagged reference from the surveillance.

One important question the user needs to deal with is how to tag a node? Can we tag any node and then access it? The answer is no, we need to ensure that the node we are about to tag is reachable from the entry point of the data structure. Otherwise, it may result in tagging of a reference which is already freed. The solution which we employ to resolve this issue is using hand-over-hand tagging and accessing\footnote{readers may worry about the number of restarts. May be a plot showing the number of restarts due to failed vreads/vwrites to pacify them?}. To do this, we maintain a rolling window like set of $k$ addresses. Inductively, a new reference could only be accessed for tagging by doing a vRead on an already tagged node. Thus, it is not possible to tag an unreachable node in hand over hand tagging without failing the vRead.

To fulfill the reclaimers rule a thread could write on the node before freeing it in one of the following ways:
\begin{itemize}
    \item Data structures can maintain a mark bit/field inside its node's structure which can be set before the node is unlinked. Or
    \item The data structure operations could unlink the node being deleted using Invalidate-and-Swap instruction proposed in MemoryTagging.
\end{itemize}

The purpose of writing on the node before deleting is to trigger invalidations of the copy of the cachelines addressed by the node at other cores. This is the part of the usual behaviour of the underlying cache coherence protocol whenever there is a write to a cacheline. Now, how does this help HBR? remember that HBR monitors the L1 cache traffic at all cores for the tagged cachlines by virtue of the readers/writers rule. If a core's L1 cache receives an invalidation request for a tagged cacheline then any subsequent access (\func{vRead}/\func{vWrite}) will fail causing therefore allowing threads at the application to know that they might access a deleted node. Thus the two rules applied together will ensure safe application of HBR to a data structure.

% HBR can be used with data structures having MemoryTagging synchronization given that other cores could invalidate the cacheline of the deleted node, if it exists. This can be achieved either by writing to the node by marking it or using an \emph{Invalidate-and-Swap}. However, if in write phase their are multiple writes then their could be a complexity (Ignored details for discussion later, food for thought: how VAS based list can do reclamation even if VAS step fails after the marking step succeeds, helping is the solution.).

% Also, HBR as a stand alone reclamation scheme can be applied to most of the existing concurrent data structures which have a long read-only \emph{traversal phase} followed by a critical section termed as an \emph{update-phase}, if they adhere to the following rules. 
% \begin{enumerate}
%     \item Every node has a mark field that is updated (set to true) before a node is freed.
%     \item Every access of shared memory locations in \emph{traversal phase} is done by vRead/vWrite and inside \emph{update phase} normal read/writes are used.
%     \item The \emph{update phase} is within locks such that locks are guaranteed to never lock freed node. 
% \end{enumerate}

In the following segment a general data structure operation design pattern using HBR where updates are done within a lock based critical section is explained.
\begin{itemize}
    \item In the traversal phase, until the operation reach a set of destination nodes, repeatedly, tag a node, vRead the node, untag the previous node. If the vRead fails then untag all the nodes and retry the search. Note, depending on the the data structure other responses to vRead failures are possible. At the end of the traversal phase a set $\mathcal{K}$ of destination nodes are identified which satisfy the following invariant: All the nodes in $\mathcal{K}$ are tagged and have been read through the successful vRead.
    
    \item Upon arriving at the update phase acquire locks on the nodes in $\mathcal{K}$. Access the nodes as appropriate to perform desired modification with regular reads/writes. Note, since it is a lock based critical section accessing the locked nodes is not vulnerable to \emph{use-after-free} therefore regular reads/writes instructions will suffice and \emph{vRead}/\emph{vWrite} are not needed. And, to free some nodes, first set their mark field and then free them following the \emph{reclaimer's} rule of writing on a node being freed.
    
    One challenge in such lock based update phase is guaranteeing that locks will not be acquired on the deleted nodes. Simplest solution is using the \emph{vRead}-\emph{vWrite} based trylock we implemented along with the HBR (\algoref{lock}). \textemdash Discuss other solutions here\textemdash.  

    \item Finally, release the locks using regular writes and untag all the S nodes.
\end{itemize}

In the following sections we provide examples of aforementioned usage pattern with a lazylist and stack. 


% \begin{algorithm}
% \caption{Put your caption here}
% \begin{algorithmic}[1]

% \Procedure{Roy}{$a,b$}       \Comment{This is a test}
%     \State System Initialization
%     \State Read the value 
%     \If{$condition = True$}
%         \State Do this
%         \If{$Condition \geq 1$}
%         \State Do that
%         \ElsIf{$Condition \neq 5$}
%         \State Do another
%         \State Do that as well
%         \Else
%         \State Do otherwise
%         \EndIf
%     \EndIf

%     \While{$something \not= 0$}  \Comment{put some comments here}
%         \State $var1 \leftarrow var2$  \Comment{another comment}
%         \State $var3 \leftarrow var4$
%     \EndWhile  \label{roy's loop}
% \EndProcedure

% \end{algorithmic}
% \end{algorithm}


\subsection{HBR with lazylist}
\textemdash Describe the tagging based trylock implementation first \textemdash.
\textemdash Describe the lazylist implementation \textemdash.
\begin{algorithm}[h]
    \caption{Using HBR with lazylist.}\label{algo:list}
    \begin{algorithmic}[1]
        \State type Node \{Key key, lock, mark, Node *next\}
        \State class Lazylist \{Node *head\}

        \Procedure{locate}{Key key}
            \State retry:
            \State pred $\leftarrow$ \crdp{head}
            \State curr $\leftarrow$ \crdp{\&pred->next} if $\bot$ \utagall{} \& retry
            \State currkey $\leftarrow$ \crdp{\&curr->key}  if $\bot$ \utagall{} \& retry
            \While{currkey < key}
                \State \utag{pred}
                \State pred $\leftarrow$ curr
                \State curr $\leftarrow$ \crdp{\&pred->next} if $\bot$ \utagall{} \& retry
                \State currkey $\leftarrow$ \crdp{\&curr->key}  if $\bot$ \utagall{} \& retry
            \EndWhile
            \State return $\langle$ pred, curr, currkey $\rangle$
        \EndProcedure
        \Statex
        \Procedure{contain}{key}
            \State $\langle$ pred, curr, currkey $\rangle$ $\leftarrow$ locate(key)
            \State \utagall{}
            \State return (currkey == key)
        \EndProcedure
    \end{algorithmic}
\end{algorithm}        

\begin{algorithm}[h]
    \caption{Using HBR with lazylist.}\label{algo:listins}
    \begin{algorithmic}[1]
        \Procedure{insert}{key}
            \State retry:
            \State $\langle$ pred, curr, currkey $\rangle$ $\leftarrow$ locate(key)
            \If{currkey == key}
                \State \utagall{} \& return False
            \EndIf
            \If{False == tryLock(\&pred->lock)}
                \State \utagall{} \& retry
            \EndIf
            \If{False == tryLock(\&curr->lock)}
                \State unlock(\&pred->lock)
                \State \utagall{} \& retry
            \EndIf
            \State node $\leftarrow$ new Node(key, curr)
            \State pred->next $\leftarrow$ node \Comment{safe. critical section. \cwr{} not needed.}
            \State unlockAll() and \utagall{}
            \State return True
        \EndProcedure
    \end{algorithmic}
\end{algorithm}        

\begin{algorithm}[h]
    \caption{Using HBR with lazylist.}\label{algo:listdel}
    \begin{algorithmic}[1]
        \Procedure{delete}{key}
            \State retry:
            \State $\langle$ pred, curr, currkey $\rangle$ $\leftarrow$ locate(key)
            \If{currkey != key}
                \State \utagall{} \& return False
            \EndIf
            \If{False == tryLock(\&pred->lock)}
                \State \utagall{} \& retry
            \EndIf
            \If{False == tryLock(\&curr->lock)}
                \State unlock(\&pred->lock)
                \State \utagall{} \& retry
            \EndIf
            \State curr->mark $\leftarrow$ true
            \State pred->next $\leftarrow$ curr->next
            \State unlockAll() \& \utagall{}
            \State free(curr)
            \State return True
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[h] 
    \caption{Tagging based lock. Precondition: Cacheline of lock should be tagged.}\label{algo:lock}
    \begin{algorithmic}[1]
        \Procedure{tryLock}{bool *lock}
            \State lockVal $\leftarrow$ \texttt{\crdp{lock}}
            \If {$\bot$ $==$ lockVal or 1 $==$ lockVal}
                \State \texttt{return 0}
            \EndIf
            \State return \cwrp{lock}{1}
        \EndProcedure

        \Statex

        \Procedure{unlock}{bool *lock}
            \State l $\leftarrow$ 0 \Comment{safe as a node can only be mutated by owner.}
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\subsection{HBR with stack}
\textemdash Describe the lazylist implementation \textemdash.

\begin{algorithm}
    \caption{Using HBR with unbounded lock free stack.}\label{algo:stack}
    \begin{algorithmic}[1]
        \State type Node \{Key key, Node *next\}
        \State class Stack \{Node *top\}

        \Procedure{push}{key}
        	\State newtop = new node(key)
            \State retry:
            \State t $\leftarrow$ \texttt{\crdp{top}}
            \If {$\bot$ == t}
                \State \texttt{untagAll() and goto retry}
            \EndIf
            \State newtop->next = t
            \If {False == \texttt{\cwrp{top}{newtop}}}
                \State \texttt{untagAll() and goto retry}
            \EndIf
        \EndProcedure
        \Statex
        \Procedure{pop}{ }
            \State retry:
            \State t $\leftarrow$ \texttt{\crdp{top}}
            \If {$\bot$ == t}
                \State \texttt{untagAll() and goto retry}
            \EndIf
            \If {NULL == t}
                \State \texttt{untagAll() and return}
            \EndIf
            \If {False == \texttt{\cwrp{top}{t->next}}}
                \State \texttt{untagAll() and goto retry}
            \EndIf
            \State free(t)
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

Discussion on API: pros and cons
\newpage
\section{Correctness}
\label{sec:corr}

safety and progress lemmas
